Neural Path Features and Neural Path Kernel : Understanding the role of gates in deep learning

Rectified linear unit (ReLU) activations can also be thought of as 'gates', which, either pass or stop their pre-activation input when they are 'on' (when the pre-activation input is positive) or 'off' (when the pre-activation input is negative) respectively. A deep neural network (DNN) with ReLU activations has many gates, and the on/off status of each gate changes across input examples as well as network weights. For a given input example, only a subset of gates are 'active', i.e., on, and the sub-network of weights connected to these active gates is responsible for producing the output. At randomised initialisation, the active sub-network corresponding to a given input example is random. During training, as the weights are learnt, the active sub-networks are also learnt, and potentially hold very valuable information. In this paper, we analytically characterise the role of active sub-networks in deep learning. To this end, we encode the on/off state of the gates of a given input in a novel 'neural path feature' (NPF), and the weights of the DNN are encoded in a novel 'neural path value' (NPV). Further, we show that the output of network is indeed the inner product of NPF and NPV. The main result of the paper shows that the 'neural path kernel' associated with the NPF is a fundamental quantity that characterises the information stored in the gates of a DNN. We show via experiments (on MNIST and CIFAR-10) that in standard DNNs with ReLU activations NPFs are learnt during training and such learning is key for generalisation. Furthermore, NPFs and NPVs can be learnt in two separate networks and such learning also generalises well in experiments.

==> abstract.tex <==
\begin{abstract}
Rectified linear unit (ReLU) activations can also be thought of as \emph{gates}, which, either pass or stop their pre-activation input when they are \emph{on} (when the pre-activation input is positive) or \emph{off} (when the pre-activation input is negative) respectively. A deep neural network (DNN) with ReLU activations has many gates, and the {on/off} status of each gate changes across input examples as well as network weights. For a given input example, only a subset of gates are \emph{active}, i.e., on, and the sub-network of weights connected to these active gates is responsible for producing the output. At randomised initialisation, the active sub-network corresponding to a given input example is random. During training, as the weights are learnt, the active sub-networks are also learnt, and could hold valuable information. 

In this paper, we analytically characterise the role of active sub-networks in deep learning. To this end, we encode the {on/off} state of the gates of a given input in a novel \emph{neural path feature} (NPF), and the weights of the DNN are encoded in a novel \emph{neural path value} (NPV). Further, we show that the output of network is indeed the inner product of NPF and NPV.  The main result of the paper shows that the \emph{neural path kernel} associated with the NPF is a fundamental quantity that characterises the information stored in the gates of a DNN. We show via experiments (on MNIST and CIFAR-10) that in standard DNNs with ReLU activations NPFs are learnt during training and such learning is key for generalisation. Furthermore, NPFs and NPVs can be learnt in two separate networks and such learning also generalises well in experiments. In our experiments, we observe that almost all the information learnt by a DNN with ReLU activations is stored in the gates - a novel observation that underscores the need to further investigate the role of gating in DNNs.
\end{abstract}


==> background.tex <==
\subsection{Background: Neural Tangent Feature and Kernel}\label{sec:background}
The neural tangent machinery was developed in some of the recent works [\citenum{ntk, arora2019exact,cao2019generalization,dudnn}] to understand optimisation and generalisation in DNNs trained using GD. For an input $x\in\R^{d_{in}}$, the \emph{neural tangent feature} (NTF) is given by $\psi_{x,\Theta}=\nabla_{\Theta}\hat{y}_{\Theta}(x)\inrdnet$, i.e.,  the gradient of the network output with respect to its weights. The \emph{neural tangent kernel} (NTK) matrix $K_{\Theta}$ on the dataset is the $n\times n$ Gram matrix of the NTFs of the input examples, and is given by $K_{\Theta}(s,s')=\ip{\psi_{x_s,\Theta},\psi_{x_{s'},\Theta}}, s,s'\in[n]$. 
\begin{proposition}[\textbf{Lemma 3.1} \cite{arora2019exact}]\label{prop:basic}
Consider the GD procedure to minimise the  squared loss $L(\Theta)=\frac{1}{2}\sum_{s=1}^n \left(\hat{y}_{\Theta}(x_s)-y_s\right)^2$ with infinitesimally small step-size: $\dot{\Theta}_t=-\nabla_{\Theta}L_{\Theta_t} $. It follows that the dynamics of the error term can be written as $\dot{e}_t=-K_{\Theta_t} e_t$. 
\end{proposition}

\textbf{Prior works} [\citenum{ntk,dudnn,arora2019exact,cao2019generalization}] have studied DNNs trained using GD in the so called `NTK regime', which occurs under appropriate randomised initialisation, and when the width of the DNN approaches infinity. The characterising property of the NTK regime is that as $w\ra\infty$, $K_{\Theta_0}\ra K^{(d)}$, and $K_{\Theta_t}\approx K_{\Theta_0}$, where $K^{(d)}$ (see \eqref{eq:ntkold} in \Cref{sec:kd}) is a deterministic matrix whose superscript $(d)$ denotes the depth of the DNN. \cite{arora2019exact} show that infinite width DNN trained using GD is equivalent to kernel regression with the limiting NTK matrix $K^{(d)}$ (and hence enjoys the generalisation ability of the limiting NTK matrix $K^{(d)}$). Further, \cite{arora2019exact} propose a pure kernel method based on what they call the CNTK, which is the limiting NTK matrix $K^{(d)}$ for an infinite width convolutional neural network (CNN). \cite{cao2019generalization} show that in the NTK regime, a DNN is almost a linear learner with the random NTFs at initialisation, and show a generalisation bound in the form of $\tilde{\mathcal{O}}\left(d\cdot\sqrt{y^\top {\left(K^{(d)}\right)}^{-1} y/n}\right)$\footnote{$a_t=\mathcal{O}(b_t)$ if $\lim\sup_{t\ra\infty}|a_t/b_t|<\infty$, and $\tilde{\mathcal{O}}(\cdot)$ is used to hide logarithmic factors in $\mathcal{O}(\cdot)$.}. 

\textbf{Open Question:} \cite{arora2019exact} report a $5\% - 6\%$ performance gain of finite width CNNs (which do not operate in the NTK regime) over the exact CNTKs corresponding to infinite width CNNs, and infer that the study of DNNs in the NTK regime cannot fully explain the success of practical neural networks yet. Can we explain the reason for the performance gain of CNNs over CNTK?

==> broad.tex <==
\section{Broader Impact}
Deep neural networks are still widely regarded as blackboxes. The standard and accepted view on the inner workings of  deep neural networks is the `layer-by-layer' viewpoint:  as the input progresses through the hidden layers, features at different levels of abstractions are learnt. This paper deviates from the standard `layer-by-layer' viewpoint, in that, it breaks down the deep neural network blackbox into its constituent paths: different set of paths get fired for different inputs, and the output is the summation of the contribution from individual paths. This makes the inner workings of deep neural networks interpretable, i.e., each input is remembered in terms of the active sub-network of the paths that get `fired' for that input, and learning via gradient descent amounts to `rewiring' of the paths. The paper also analytically connects this sub-network and path based view to the recent kernel based interpretation of deep neural networks, and furthers the understanding of feature learning in deep neural networks. We believe that these better insights into the working of DNNs  can potentially lead to foundational algorithmic development in the future.



==> contrib.tex <==
\subsection{Our Contributions}\label{sec:contrib}
To the best of our knowledge, we are the first to analytically characterise the role played by active sub-networks in deep learning as presented in the `Claims I and II'.  The key contributions can be arranged into three landmarks as described below.

$\bullet$ The first step involves breaking a DNN into individual paths, and each path again into gates and weights.  To this end, we encode the states of the gates in a novel \emph{neural path feature} (NPF) and the weights in a novel \emph{neural path value} (NPV) and express the output of the DNN as an inner product of NPF and NPV (see \Cref{sec:path}). In contrast to NTF/NTK which are \emph{first-order} quantities (based on derivatives with respect to the weights), NPF and NPV are \emph{zeroth-order} quantities. The kernel matrix associated to the NPFs namely the \emph{neural path kernel} (NPK) matrix $H_{\Theta}\in\R^{n\times n}$ has a special structure, i.e., it can be written as a \emph{Hadamard} product of the input Gram matrix, and a correlation matrix $\Lambda_{\Theta}\in\R^{n\times n}$, whose entries $\Lambda_{\Theta}(s,s')$ is equal to the total number of path in the sub-network that is active for both input examples $s,s'\in[n]$. With the $\Lambda_{\Theta}$ matrix we reach our first landmark.

$\bullet$  Second step is to characterise performance of active sub-networks in a `stand alone' manner. To this end, we consider a new idealised setting namely fixed NPF (FNPF) setting, wherein, the NPFs are fixed (i.e., held constant) and only the NPV is learnt via gradient descent. In this setting, we show that (see \Cref{th:main}), in the limit of infinite width and under randomised initialisation the NTK converges to a matrix $K^{(d)}_{\text{FNPF}}=\text{constant} \times H_{\text{FNPF}}$, where $H_{\text{FNPF}}\in\R^{n\times n}$ is the NPK matrix corresponding to the fixed NPFs. $K^{(d)}$ matrix of \cite{ntk,arora2019exact,cao2019generalization} becomes the $K^{(d)}_{\text{FNPF}}$ matrix in the FNPF setting,  wherein, we initialise the NPV statistically independent of the fixed NPFs (see \Cref{th:main}). With \Cref{th:main}, we reach our second landmark, i.e. we justify ``Claim I'', that active sub-networks are fundamental entities, which follows from the fact that $H_{\text{FNPF}}=\Sigma\odot \Lambda_{\text{FNPF}}$, where $\Lambda_{\text{FNFP}}$ corresponds to the fixed NPFs.

$\bullet$ Third step is to show experimentally that sub-network learning happens in practice. We show that in finite width DNNs with ReLU activations, NPFs are learnt continuously during training, and such learning is key for generalisation. We observe that fixed NPFs obtained from the initial stages of training generalise poorly than CNTK (of \cite{arora2019exact}), whereas, fixed NPFs obtained from later stages of training generalise better than CNTK and generalise as well as standard DNNs with ReLU. This throws light on the open question in \Cref{sec:background}, i.e., the difference between the NTK regime and the finite width DNNs is perhaps due to NPF learning. In finite width DNNs, NPFs are learnt during training and in the NTK regime no such feature learning happens during training (since $K^{(d)}$ is fixed). Since the NPFs completely encode the information pertaining to the active sub-networks, we complete our final landmark namely  justification of ``Claim II'', 

==> decoupled.tex <==
\section{Deep Gated Networks: Decoupling Neural Path Feature and Value}\label{sec:decoupled}
The next step towards our goal of understanding the role of the gates (and gate dynamics) is the separation of the gates i.e., the NPFs from the weights, i.e., the NPV.  This is achieved by a deep gated network (DGN) having two networks of identical architecture namely i) a feature network parameterised by $\Tf\in\R^{\dfnet}$, that holds gating information, and hence the NPFs and ii) a value network that holds the NPVs parameterised by $\Tv\in\R^{\dvnet}$. As shown in \Cref{fig:dgn}, the gates/NPFs are generated in the feature network and are used in the value network. In what follows, we let $\Tdgn=(\Tf,\Tv)\in\R^{\dfnet+\dvnet}$to denote the combined parameters of a DGN. 
\begin{figure}[t] 
\begin{minipage}{0.79\columnwidth}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|  l | l |}\hline
 Feature Network (NPF)& Value Network (NPV)\\
 $z^{\text{f}}_{x}(0)=x$ &$z^{\text{v}}_{x}(0)=x$ \\
$q^{\text{f}}_{x}(i,l)=\sum_{j} \Tf(i,j,l)\cdot z_{x}(j,l-1)$ & $q^{\text{v}}_{x}(i,l)=\sum_{j} \Tv(i,j,l)\cdot z^{\text{v}}_{x}(j,l-1)$\\
$z^{\text{f}}_{x}(i,l)= q^{\text{f}}_{x}(i,l)\cdot\mathbbm{1}_{\{q^{\text{f}}_{x}(i,l)>0\}}$& $z^{\text{v}}_{x}(i,l)= q^{\text{v}}_{x}(i,l)\cdot G_{x}(i,l)$ \\
 None &$\hat{y}_{\Tdgn}(x)= \sum_{j} \Tv(1,j,l)\cdot z^{\text{v}}_{x}(j,d-1)$\\\hline
\multicolumn{2}{|l|}{{Hard ReLU: $G_{x}(i,l)=\mathbbm{1}_{\{q^{\text{f}}_{x}(i,l)>0\}}$ or Soft-ReLU: $G_{x}(i,l)={1}/{\left(1+\exp(-\beta\cdot q^{\text{f}}_{x}(i,l)>0)\right)} $}}\\\hline
\end{tabular}
}
\end{minipage}
\begin{minipage}{0.20\columnwidth}
\resizebox{\columnwidth}{!}{
\includegraphics[scale=0.4]{figs/dgn.png}
}
\end{minipage}
\caption{Deep gated network (DGN) setup.  The pre-activations $q^{\text{f}}_{x}(i,l)$ from the feature network are used to derive the gating values $G_{x}(i,l)$. }
\label{fig:dgn}
\end{figure}

\textbf{Regimes of a DGN:} We can configure the DGN in four different \emph{regimes} by controlling (i)  the trainability of $\Tf$, and (ii) the initialisation of $\Tf_0$. By setting $\Tf$ to be \emph{non-trainable/trainable} we can compare fixed NPFs and NPFs that change during training. By setting $\Tf_0$ to be \emph{random/pre-trained} we can compare random NPFs and learnt NPFs. By setting $\Tf_0=\Tv_0$ we can mimic the initialisation of a standard DNN with ReLU. The four regimes of a DGN are described below (note that in all the regimes $\Tv$ is trainable and $\hat{y}_{\Tdgn}$ is the output node).

1. Decoupled Learning of NPF (DLNPF): Here, $\Tf$ is trainable, and hence the NPFs are learned in a decoupled manner (as opposed to the standard DNN with ReLU where a single parameter is responsible for learning NPFs and NPV). Here, soft-ReLU with $\beta>0$ is used to ensure gradient flow via feature network. $\Tf_0,\Tv_0$ are initialised at random and are statistically independent.

2. Fixed Learnt NPF (FLNPF): Here $\Tf$ is non-trainable, and $\Tf_0$ copied from a  pre-trained network (i.e., NPFs are fixed and learnt). $\Tv_0$ are initialised at random and is statistically independent of $\Tf_0$.

3. Fixed Random NPF with Independent Initialisation (FRNPF-II): Here,  $\Tf_0,\Tv_0$ are initialised at random are statistically independent. Also, $\Tf$ is non-trainable, i.e.,  the NPFs are random and fixed.

4. Fixed Random NPF with Dependent Initialisation (FRNPF-DI):  Here, the initialisation mimics standard DNN with ReLU, i.e., $\Tf_0=\Tv_0$ are initialised at random, and $\Tf$ is non-trainable.

\textbf{Remark:} The DGN and its regimes are idealised models to understand the role of gates, and not alternate proposals to replace standard DNNs with ReLU activations. 
\begin{proposition}[Gradient Dynamics in a DGN]\label{prop:dgn} Let $\psif_{x,\Tdgn}\stackrel{def}=\nabla_{\Tf}\hat{y}_{\Tdgn}(x) \in \R^{\dfnet}$, $\psiv_{x,\Tdgn}\stackrel{def}=\nabla_{\Tv}\hat{y}_{\Tdgn}(x) \in \R^{\dvnet}$. Let $K^{\text{v}}_{\Tdgn}$ and $K^{\text{f}}_{\Tdgn}$ be $n\times n$ matrices with entries $K^{\text{v}}_{\Tdgn}(s,s')=\ip{\psiv_{x_s,\Tdgn},\psiv_{x_{s'},\Tdgn}}$ and $K^{\text{f}}_{\Tdgn}(s,s')=\ip{\psif_{x_s,\Tdgn},\psif_{x_{s'},\Tdgn}}$. For infinitesimally small step-size of GD, the error dynamics in a DGN (in the DLNPF and FNPF modes) is given by:
\FloatBarrier
\begin{table}[h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{| l | l l l | l |}\hline
	Dynamics&		&&Decoupled Learning& Fixed NPF\\\hline
		&		&&& \\
Weight  & $\dot{\Theta}^{\text{v}}_t$&$=$&$-\sum_{s=1}^n \psiv_{x,\Tdgn_t}e_t(s),\dot{\Theta}^{\text{f}}_t=-\sum_{s=1}^n \psif_{x,\Tdgn_t}e_t(s)$ & $\dot{\Theta}^{\text{v}}_t$ same as (DLNFP),  $\dot{\Theta}^{\text{f}}_t=0$\\
NPF & $\dot{\phi}_{x_s,\Tf_t}(p)$&$=$&$x(\I_0(p))\sum_{\Tf\in\Tf}\partial_{\Tf}A_{\Tf_t}(x_s,p)\dot{\theta}^{\text{f}}_t,\forall p\in[P], s\in[n]$& $\dot{\phi}_{x_s,\Tf_t}(p)=0$\\
NPV & $\dot{v}_{\Tv_t}(p)$&$=$&$\sum_{\tv\in\Tv}\partial_{\tv}v_{\Tv_t}(p)\dot{\theta}^{\text{v}}_t,\forall p\in[P]$ & $\dot{v}_{\Tv_t}(p)$ same as DLNPF\\
Error & $\dot{e}_t$&$=$&$-\left(K^{\text{v}}_{\Tdgn}+ K^{\text{f}}_{\Tdgn}\right)e_t$  & $\dot{e}_t=-\left(K^{\text{v}}_{\Tdgn}\right)e_t$ \\\hline
\end{tabular}
}
\end{table}
\end{proposition}
\textbf{Remark:} The gradient dynamics in a DGN specified in \Cref{prop:dgn} is similar to the gradient dynamics in a DNN specified in \Cref{prop:dnnhard}. Important difference is that (in a DGN) the NTF $\psi_{x,\Theta}=(\psif_{x,\Theta},\psiv_{x,\Theta})\in\R^{\dfnet+\dvnet}$, wherein, $\psiv_{x,\Tdgn}\in\R^{\dvnet}$ and $\psif_{x,\Tdgn}\in\R^{\dfnet}$ flow through the value and feature networks respectively. Here, NPF learning is captured explicitly by $\psif$ and $\kf$. 

==> experiments.tex <==
\section{Experiments: Fixed NPFs, NPF Learning and Verification of Claim II}\label{sec:experiments} 
In this section, we experimentally investigate the role of gates and empirically justify ``Claim II'', i.e., learning of the active sub-networks improves generalisation.  In our framework, since the gates are encoded in the NPFs, we justify ``Claim II'' by showing that NPF learning improves generalisation. For this purpose, we make use of the DGN setup and its four different regimes.  We show that NPF learning also explains the performance gain of finite width CNN over the pure kernel method based on the exact infinite width CNTK. We now describe the setup and then discuss the results.
\subsection{Setup}
\textbf{Datasets:} We used standard datasets namely MNIST and CIFAR-10, with categorical cross entropy loss. We also used a `Binary'-MNIST dataset (with squared loss), which is MNIST with only the two classes corresponding to digits $4$ and $7$, with label $-1$ for digit $4$ and $+1$ for digit $7$.

\textbf{Optimisers:} We used stochastic gradient descent (SGD) and \emph{Adam} as optimisers. In the case of SGD, we tried constant step-sizes in the set $\{0.1,0.01,0.001\}$ and chose the best. In the case of Adam the we used a constant step size of $3e^{-4}$. In both cases, we used batch size to be $32$.  

\textbf{Architectures:} For MNIST we used fully connected (FC) architectures with $(w=128,d=5)$. For CIFAR-10, we used a \emph{`vanilla' convolutional} architecture namely VCONV and a \emph{convolutional} architecture with \emph{global-average-pooling} (GAP) namely GCONV. GCONV had no pooling, residual connections, dropout or batch-normalisation, and is given as follows: input layer is $(32, 32, 3)$, followed by $4$ convolution layers, each with a stride of $(3, 3)$ and channels $64$, $64$, $128$, $128$ respectively. The convolutional layers are followed by GAP layer, and a FC layer with $256$ units, and a soft-max layer to produce the final predictions. VCONV is same as GCONV without the (GAP) layer.

\begin{comment}
The performance of the following networks on standard MNIST and CIFAR-10 datasets will be used for comparison: (i) fixed random (FRNPF): in the DGN, we randomly initialise both $\Tf_0,\Tv_0$, make $\Tf$ \emph{non-trainable} and train only $\Tv$ , (ii) fixed learnt (FLNPF): we initialise $\Tv_0$ randomly, and copy weights from a pre-trained ReLU network (of identical architecture) into $\Tf_0$. Similar to FR case, $\Tf$ is non-trainable and only $\Tv$ is trained (iii) decoupled learning (DLNPF):  we randomly initialise both $\Tf_0,\Tv_0$, and train both $\Tf$ and $\Tv$, (iv) ReLU: Standard DNNs/CNNs with ReLU.  We will also use the numerical results reported in \cite{arora2019exact}.\\
\end{comment}
 \begin{table}[t]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}\hline
Arch			&Optimiser	&Dataset		&FRNPF (II) 			&FRNPF (DI)			&DLNPF					&FLNPF						&ReLU\\\hline
FC			&SGD		&MNIST 		&$95.85\pm0.10$		&$95.85\pm0.17$		&$97.86\pm0.11$			&$97.10\pm0.09$				&$97.85\pm0.09$\\\hline
FC			&Adam		&MNIST 		&$96.02\pm0.13$		&$96.09\pm0.12$		&$\mathbf{98.22\pm0.05}$	&$\mathbf{97.82\pm0.02}$		&$\mathbf{98.14\pm0.07}$\\\hline
VCONV		&SGD		&CIFAR-$10$	&$58.92\pm0.62$		&$58.83\pm0.27$ 		&$63.21\pm0.07$			&$63.06\pm0.73$				&$67.02\pm0.43$\\\hline
VCONV		&Adam		&CIFAR-$10$	&$64.86\pm1.18$		&$64.68\pm0.84$		&$\mathbf{69.45\pm0.76}$	&$\mathbf{71.4\pm0.47}$			&$\mathbf{72.43\pm0.54}$\\\hline
GCONV	&SGD		&CIFAR-$10$	&$67.36\pm0.56$		&$66.86\pm0.44$		&$\mathbf{74.57\pm0.43}$			&$\mathbf{78.52\pm0.39}$				&$\mathbf{78.90\pm0.37}$\\\hline
GCONV	&Adam		&CIFAR-$10$	&$67.09\pm0.58$		&$67.08\pm0.27$		&$\mathbf{77.12\pm0.19}$	&$\mathbf{79.68\pm0.32}$		&$\mathbf{80.43\pm0.35}$\\\hline
\end{tabular}
}
\caption{Shows the test accuract of different NPFs learning settings. Each model is trained close to $100\%$. In each run, the best test accuracy is taken and the table presents values averaged over $5$ runs.
}
\label{tb:npfs}
\end{table}
\normalsize
\subsection{Result Discussion}
$1.$ \textbf{Decoupling:} There is no significant performance difference between FRNPF-II and FRNPF-DI regimes, i.e., the statistical independence of $\Tv_0$ and $\Tf_0$ did not affect performance. Also, DLNPF performed better than FRNPF, which shows the that NPFs can also be learned in a decoupled manner.

$2.$ \textbf{Performance gain of CNN over CNTK} can be explained by NPF learning. For this purpose, we look at the performance of GCONV models trained with \emph{Adam} on CIFAR-10 (last row of \Cref{tb:npfs}). Consider models grouped as $S_1=\{$FRNPF-DI,FRNPF-II$\}$, $S_2=\{$CNTK$\}$ that have no NPF learning versus models grouped as $S_3=\{$DLNPF, FLNPF, ReLU$\}$ that have either NPF learning during training or a fixed learnt NPF. The group $S_3$ performs better than $S_1$ and $S_2$. Note that, both $S_1$ and $S_3$ are finite width networks, yet, performance of $S_1$ is worse than CNTK, and the performance of $S_3$ is better than CNTK. Thus finite width alone does not explain the performance gain of CNNs over CNTK. Further, all models in group $S_3$ are finite width and also have NPF learning. Thus, finite width together with NPF learning explains the performance gain of CNN over CNTK.

$3.$ \textbf{Standard features vs NPFs:} The standard view is that the outputs of the intermediate/hidden layers learn lower to higher level features (as depth proceeds) and the final layer learns a linear model using the hidden features given by the penultimate layer outputs. This view of feature learning holds true for all the models in $S_1$ and $S_3$. However, only NPF learning clearly \emph{discriminates} between the different regimes $S_1, S_2$ and $S_3$. Thus, NPF learning is indeed a unique aspect in deep learning.

$4.$ \textbf{Continuous NPF Learning:} The performance gap between FRNPF and ReLU is continuous. In the case of CIFAR-10, we trained a GCONV network (parameterised by $\bar{\Theta}$) for $60$ epochs, and we obtained $6$ different weights at various \emph{stages} of the training process. Stage $i$: $\bar{\Theta}_{10\times i}, i=1,\ldots,6$. We copied these weights obtained at various stages of training to setup $6$ different FLNPFs, i.e., FLNPF-$1$ to FLNPF-$6$. We observe that the performance of FLNPF-$1$ to FLNPF-$6$ increases monotonically, with FLNPF-$1$ performing $72\%$ which is better than FRNPF (i.e., $67.08\%$),  and FLNPF-$6$ performing as well as ReLU (see left most plot in \Cref{fig:dynamics}). The performance of CNTK of \cite{arora2019exact} is $77.43\%$. Thus, through its various stages, the FLNPF starts from below $77.43\%$ and surpasses to reach $79.68\%$, which implies performance gain of CNN is due to learning of NPFs.

\begin{figure}[h]
\centering
\includegraphics[scale=0.23]{figs/gap.png}
\includegraphics[scale=0.23]{figs/path-gram.png}
\includegraphics[scale=0.23]{figs/kvkphi.png}
\caption{Dynamics of NPF Learning. }
\label{fig:dynamics}
\end{figure}


$5.$ \textbf{Dynamics of active sub-networks during training:} We considered ``Binary''-MNIST data set with two classes namely digits $4$ and $7$, with the labels taking values in $\{-1,+1\}$ and squared loss. We trained a fully connected (FC) network ($w=100$, $d=5$). Let $\widehat{H}_{\Theta_t}=\frac{1}{trace(H_{\Theta_t})}H_{\Theta_t}$ be the normalised NPK matrix. For a subset size, $n'=200$ ($100$ examples per class) we plot $\nu_t=y^\top (\widehat{H}_{\Theta_t})^{-1} y$, (where $y\in\{-1,1\}^{200}$ is the labelling function), and observe that $\nu_t$ reduces as training proceeds (see middle plot in \Cref{fig:dynamics}). Note that, $\nu_t=\sum_{i=1}^{n'}(u_{i,t}^\top y)^2 (\hat{\rho}_{i,t})^{-1}$, where $u_{i,t}\in \R^{n'}$ are the orthonormal eigenvectors of $\widehat{H}_{\Theta_t}$ and $\hat{\rho}_{i,t},i\in[n']$ are the corresponding eigenvalues. Since $\sum_{i=1}^{n'}\hat{\rho}_{i,t}=1$, the only way $\nu_t$ reduces is when more and more energy gets concentrated on $\hat{\rho}_{i,t}$s for which $(u_{i,t}^\top y)^2$s are also high. Since $H_{\Theta_t}=\Sigma\odot \Lambda_{\Theta_t}$, only $\Lambda_{\Theta_t}$ is learnt during training.

$6.$ \textbf{How are NPFs learnt?} In order to understand this, in the case of DNNs with ReLU, we can replace the hard-ReLU gate by soft-ReLU gate. Now, the gradient of the output is given $\partial_{\theta}\hat{y}_{\Theta}(x)=\ip{\partial_{\theta} \phi_{x,\Theta},v_{\Theta}}+\ip{\phi_{x,\Theta},\partial_{\theta} v_{\Theta}}$, where the two terms on the right can be interpreted as NPF and NPV gradients. The advantage of using soft-ReLU is that $\psif\neq 0$ (note that $\psif=0$ for hard-ReLU due to their $0/1$ state). We can obtain further insights in the DLNPF regime, wherein, the NTK is given by $K_{\Tdgn}=K^{\text{v}}_{\Tdgn}+K^{\text{f}}_{\Tdgn}$. For MNIST, we compared $K^{\text{v}}_{\Tdgn}$ and $K^{\text{f}}_{\Tdgn}$ (calculated on $100$ examples in total with $10$ examples per each of the $10$ classes) using their trace and Frobenius norms, and we observe that $K^{\text{v}}_{\Tdgn}$ and $K^{\text{f}}_{\Tdgn}$ are in the same scale (see right plot in \Cref{fig:dynamics}), which perhaps shows that both $K^{\text{f}}_{\Tdgn}$ and $K^{\text{f}}_{\Tdgn}$ are equally important for obtaining good generalisation performance. Studying $K^{\text{f}}_{\Tdgn}$ responsible for NPF learning is an interesting future research direction.



==> future.tex <==
\section{Conclusion}
\begin{comment}
Optimisation and generalisation of DNNs has been an important question in machine learning. Prior works have considered the \emph{neural tangent features} (NTF) and an associated \emph{neural tangent kernel} (NTK), which are quantities based on the first-order gradient information.  In this paper, we looked at fully connected DNNs with ReLU activations, and for such networks, we defined a novel feature namely the \emph{neural path feature} (NPF) and an associated \emph{neural path kernel} , which are \emph{zeroth-order} quantities. The NPFs are based on the information in the gates of a DNN, and hence the NPFs change as the network is trained. We theoretically showed that NPK can be used to understand the optimisation and generalisation for models trained with fixed NPFs. We showed in the experiments that in standard DNNs with ReLU activations, NPFs are learnt during training, and such NPF learning is key for generalisation performance. We also showed via experiments that deep gated networks, where NPFs are learned in a decoupled manner also generalise well. 

A possible future direction is to understand the role of depth and width in NPF learning, and the role of NPF in generalisation. The deep gated network might be useful in this effort, since the NPFs learning is decoupled and is perhaps amenable to analysis in comparison the standard DNNs.
\end{comment}
In this paper, we studied the role of active sub-networks in deep learning by encoding the gates in the neural path features. We showed that the neural path features are learnt during training and such learning is key for generalisation. In our experiments, we observed that almost all information of a trained DNN is stored in the neural path features. We conclude by saying that \emph{understanding deep learning requires understanding neural path feature learning}. %The deep gated network whose gates are decoupled is perhaps an easier starting point to analyse neural path feature learning. 
%A possible future direction is to understand the role of depth and width in NPF learning, and the role of NPF in generalisation.
\begin{comment}
In this paper, we considered the problem of optimisation and generalisation in DNNs with ReLU activations. Throughout the paper, we exploited the special property of the ReLU activation, in that, i output of a ReLU activation be expressed as a product of its pre-activation input and its gating value which is $1/0$ based on whether or not the pre-activation is positive or negative. To analyse such networks, we  introduced the `path-view': a path starts from the input passes through one weight and one hidden nodes per layer and finally ends in the output, and the output of a network is seen as a cumulative combination of the contributions from various paths. The computation in each path was further divided into those happening in the weights, and those happening in the gates. This enabled us to express the output of such DNNs as an inner product of neural path feature (for a path, its feature is the product of gates it encounters from input to output)  and neural path value (for a path, its value is the product of weights it encounters from input to output). The neural path feature (NPF) of a given input is completely dictated by the gating pattern, i.e., the \emph{on/off} status of the gates in the network for that input. Due to the \emph{on/off} nature of the gates, their change to infinitesimal change in the network parameters is $0$, i.e., the gradient of the NPFs with respect to the network weights is $0$. However, in practice the NPFs change during training. By considering a soft-ReLU activation, which served as a `differentiable' substitute for the ReLU activation, we could capture the feature gradient, i.e., the gradient of the NPFs with respect to the network weights. This enabled us to write down the gradient descent dynamics that incorporated NPF learning. We presented the following interesting results:

$1.$ In the fixed NPF regime, wherein, the NPFs are held constant through training, the optimisation and generalisation depends on the associated neural path kernel.

$2.$ 
\end{comment}


==> gatedyna.tex <==
\section{Dynamics of Gradient Descent with NPF and NPV Learning}\label{sec:gatedyna}
In \Cref{sec:path}, we mentioned that during gradient descent, the DNN is learning a relation $\hat{y}_{\Theta}(x)=\ip{\phi_{x,\Theta}, v_{\Theta}}$, i.e., both the NPFs and the NPV are learned during gradient descent. In this section, we connect the newly defined quantities, i..e, NPFs and NPV to the NTK matrix $K_{\Theta}$ (see \Cref{prop:ntknew}), and re-write the gradient descent dynamics in \Cref{prop:dnnhard}.
\subsection{Dynamics of NPFs and NPV}
\begin{definition}\label{def:npvgrad}
The gradient of the NPV of path $p$ is defined as $\varphi_{p,\Theta}\stackrel{def}=(\partial_{\theta}v_{\Theta}(p), \theta \in\Theta)\in\R^{d_{net}}$.
\end{definition}
\textbf{Remark} The change of the NPV is given by $\dot{v}_{\Theta_t}(p)=\ip{\varphi_{p,\Theta_t},\dot{\Theta}_t}$, where $\dot{\Theta}_t$ is the change of the weights. We now collect the gradients $\varphi_{p,\Theta}$ of all the paths to define a \emph{value tangent kernel} (VTK). 
\begin{definition}
Let $\nabla_{\Theta}v_{\Theta}$ be a $d_{net}\times P$ matrix of NPV derivatives given by $\nabla_{\Theta}v_{\Theta}=(\varphi_{p,\Theta},p\in[P])$. Define the VTK to be the $P\times P$ matrix given by $\V_{\Theta}=(\nabla_{\Theta}v_{\Theta})^\top(\nabla_{\Theta}v_{\Theta})$.
\end{definition}
\textbf{Remark} An important point to note here is that the VTK is a quantity that is dependent only on the weights. To appreciate the same, consider a deep linear network (DLN) [\citenum{shamir,dudln}] which has identity activations, i.e., all the gates are $1$ for all inputs, and weights. For a DLN and DNN with identical network architecture (i.e., $w$ and $d$), and identical weights, $\V_{\Theta}$ is also identical. Thus, $\V_{\Theta}$ is the gradient based information that excludes the gating information.

The NPFs changes at those time instants when any one of the gates switches from $1$ to $0$ or from $0$ to $1$. In the time between two such switching instances, NPFs of all the input examples in the dataset remain the same, and between successive switching instances,  the NPF of at least one of the input example in the dataset changes. In what follows, in \Cref{prop:dnnhard} we re-write \Cref{prop:basic} taking into account the switching instances which we define in \Cref{def:switch}.
\begin{definition}\label{def:switch}
Define a sequence of monotonically increasing time instants $\{T_{i}\}_{i=0}^\infty$ (with $T_0=0$) to be `switching' instants if $\phi_{x_s,\Theta_t}=\phi_{x_s,\Theta_{T_i}},\forall s\in[n],\forall t\in[T_{i},T_{i+1}), i=0,\ldots,\infty$, and  $\forall i=0,\ldots, \infty$ $\exists s(i)\in[n]$ such that $\phi_{x_{s(i)},\Theta_{T_i}}\neq \phi_{x_{s(i)},\Theta_{T_{i+1}}}$.
\end{definition}
\subsection{Re-writing Gradient Descent Dynamics}
\begin{proposition}\label{prop:ntknew}
The NTK is given by $K_{\Theta}=\Phi^\top_{\Theta}\V_{\Theta}\Phi_{\Theta}$.
\end{proposition}
\textbf{Remark} $K_{\Theta_t}$ changes during training (i) continuously at all $t\geq 0$ due to $\V_{\Theta_t}$, and (ii) at switching instants $T_{i},i=0,\ldots,\infty$ due to the change in $\Phi_{\Theta_{T_i}}$. We now describe the gradient descent dynamics taking into the dynamics of the NPV and the NPFs.
\begin{proposition}\label{prop:dnnhard}
Let $\{T_i\}_{i=0}^\infty$ be as in \Cref{def:switch}. For $t\in[T_{i},T_{i+1})$ and small step-size of GD:
\FloatBarrier
\begin{table}[h]
\centering
\begin{tabular}{ l c l l l }
Weights Dynamics &:  & $\dot{\Theta}_t$&$=$&$-\sum_{s=1}^n \psi_{x_s,\Theta_t}e_t(s)$\\
NPV Dynamics&: & $\dot{v}_{\Theta_t}(p)$&$=$&$\ip{\varphi_{p,\Theta_t},\dot{\Theta}_t},\forall p\in[P]$\\
Error Dynamics&: & $\dot{e}_t$&$=$&$-K_{\Theta_t}e_t$, where $K_{\Theta_t}=\Phi^\top_{\Theta_{T_i}}\V_{\Theta_t}\Phi_{\Theta_{T_i}}$\\
\end{tabular}
\end{table}
\end{proposition}
\begin{proposition}\label{prop:condition}
Let the maximum and minimum eigenvalues of a real symmetric matrix $A$ be denoted by $\rho_{\max}(A)$ and $\rho_{\min}(A)$. Then, $\rho_{min}(K_{\Theta})\leq \rho_{\min}(H_{\Theta})\rho_{\max}\left(\V_{\Theta}\right)$.
\end{proposition}
\textbf{Remark} For the NTK to be well conditioned, it is necessary for the NPK to be well conditioned. This is intuitive, in that, the closer two inputs are, the closer are their NPFs, and it is harder to train the network to produce arbitrarily different outputs for such inputs that are very close to one another.

==> infomeasure.tex <==
\section{Learning with Fixed NPFs: Role Of Active Sub-Networks}\label{sec:infomeasure}
We now show that in the fixed NPF regime, at randomised initialisation, $\text{NTK}=\text{const}\times\text{NPK}$. Due to the \emph{Hadamard} structure of the NPK (\Cref{lm:npk}) it follows that the active sub-networks are fundamental entities in DNNs (theoretically justifying  ``Claim I''). 
\begin{theorem} \label{th:main} Let $H_{\text{FNFP}}$ refer to $H_{\Tf_0}$. Let (i) $\Tv_0\inrdnet$ is statistically independent of  $\Tf_0\inrdnet$, and (ii) $\Tv_0$ are sampled i.i.d from symmetric Bernoulli over $\{-\sigma,+\sigma\}$. For $\sigma=\frac{\sigma'}{w}$,  \begin{align*}K^{\text{v}}_{\Tdgn_0}\ra K^{(d)}_{\text{FNPF}} =d\cdot \sigma^{2(d-1)} \cdot H_{\text{FNPF}},  \,\text{as}\, w\ra\infty\end{align*}
\end{theorem}
$\bullet$ \textbf{Statistical independence} of $\Tf_0$ and $\Tv_0$ assumed in \Cref{th:main} holds only for the three regimes namely DLNPF, FLNPF, FRNPF-II. However, in DNN with ReLU (and also in FRNPF-DI) $\Tf_0=\Tv_0$, and hence the assumption in \Cref{th:main} does not capture the conditions at initialisation of a standard DNN. At the same time, it is important to note that the current state-of-the-art analysis for DNNs is in the infinite width regime \cite{ntk,arora2019exact,cao2019generalization}, wherein, the activations undergo only an order of $\frac{1}{\sqrt{w}}$ change during training. Since $\frac{1}{\sqrt{w}}\ra 0$, as $w\ra\infty$, the assumption that the NPFs (i.e., gates) remain fixed during training is not a strong one. Once the NPFs are fixed, statistical independence of $\Tv_0$ is a natural choice. Also, we do not observe significant empirical difference between the FRNPF-DI and FRNPF-II regimes (see \Cref{sec:experiments}).

$\bullet$ \textbf{Role of active sub-networks:} Thanks to the statistical independence of $\Tf_0$ and $\Tv_0$, $K^{(d)}$ in prior works [\citenum{ntk,arora2019exact,cao2019generalization}] essentially becomes $K^{(d)}_{\text{FNPF}}$ in \Cref{th:main}.  From previous results \cite{arora2019exact}, it follows that as $w\ra\infty$, the optimisation and generalisation properties of the fixed NPF learner can be tied down to the infinite width NTK of the FNPF learner $K^{(d)}_{\text{FNPF}}$ and hence to $H_{\text{FNPF}}$ (treating $d\sigma^{2(d-1)}$ as a scaling factor).  We can further breakdown $H_{\text{FNPF}}=\Sigma\odot{\Lambda}_{\text{FNPF}}$, where $\Lambda_{\text{FNPF}}=\Lambda_{\Tf_0}$. This justifies ``Claim I''. We also observe in our experiments that using the learnt NPFs (i.e., in the FLNPF regime), we can reset and re-train the NPV without significant loss of performance, a fact that underscores the importance of the NPFs and the active sub-networks.

 $\bullet$ \textbf{Scaling factor:} The scaling factor $d$ is due to the fact that in a path there are $d$ weights and the sensitivity of each weight is $\sigma^{(d-1)}$. In the case of random NPFs obtained by initialising $\Tf_0$ at random by sampling from a symmetric distribution, we expect $\frac{w}2$ gates to be on every layer, so $\sigma=\sqrt{\frac{2}{w}}$ is a normalising choice, in that, the diagonal entries of $\sigma^{2(d-1)}{\Lambda}_{\text{FNPF}}(s,s)\approx 1$ in this case.

$\bullet$ We discuss a more detailed version of \Cref{th:main} in the Appendix, where we discuss the role of width and depth on a pure memorisation task.


==> intro.tex <==
\section{Introduction}
We consider deep neural networks (DNNs) with rectified linear unit (ReLU) activations. A special property of the ReLU activation (denoted by $\chi$) is that its output can be written as a product of its pre-activation input, say $q\in\R$ and a gating signal, $G(q)=\mathbbm{1}_{\{q>0\}}$, i.e., $\chi(q)=q\cdot G(q)$. While the weights (of a DNN) remain the same across input examples, the $1/0$ state of the gates (or simply gates) change across input examples. For each input example, there is a corresponding \emph{active sub-network} consisting of those gates which are $1$, and the weights which pass through such gates. This active sub-network can be said to hold the memory for a given input, i.e., only those weights that pass through such active gates contribute to the output. In this viewpoint, at random initialisation of the weights, for a given input example, a random sub-network is active and produces a random output.  However, as the weights change during training (say using gradient descent), the gates change, and hence the active sub-networks also change
corresponding to the various input examples also change. At the end of training, for each input example, there is a learned active sub-network, and produces a learned output. Thus, the gates of a trained DNN could potentially contain valuable information. 

We focus on DNNs with ReLU activations. The goals and claims in this paper are state below.\\
\begin{tabular}{lll}
Goal &:& \emph{Study the role of the gates in DNNs trained with gradient descent (GD).}\\
Claim I (\Cref{sec:infomeasure})  &:& \emph{Active sub-networks are fundamental entities.}  \\
Claim II (\Cref{sec:experiments})	&:& \emph{Learning of the active sub-networks improves generalisation.}
\end{tabular}

Before we discuss the claims in terms of our novel technical contributions in \Cref{sec:contrib}, we present the background of  \emph{neural tangent} framework in \Cref{sec:background}.

\textbf{Notation:} We denote the set $\{1,\ldots, n\}$ by $[n]$. For $x,y\in\R^m$, $\ip{x,y}=x^\top y$. The dataset is denoted by $(x_s,y_s)_{s=1}^n\in\R^{\din}\times \R$. For an input $x\in\R^{\din}$, the output of the DNN  is denoted by $\hat{y}_{\Theta}(x)\in\R$, where $\Theta\in\R^{\dnet}$ are the weights. We use $\theta\in\Theta$ to denote single arbitrary weight, and $\partial_{\theta}(\cdot)$ to denote $\frac{\partial (\cdot)}{\partial \theta}$. We use $\nabla_{\Theta}(\cdot)$ stands for the gradient of $(\cdot)$ with respect to the network weights. We use vectorised notations $y=(y_s,s\in[n]), \hat{y}_{\Theta}=\left(\hat{y}_{\Theta}(x_s), s\in[n]\right)\in\R^n$ for the true and predicted outputs and $e_{t}= (\hat{y}_{\Theta_t}-y)\in\R^n$ for the error in the prediction.


\input{background}
\input{contrib}

==> motivation.tex <==
\section{ Role of Gates: Motivation }
In this paper, we take the `path-view': the output of a DNN is obtained as a summation of the contribution of individual paths, which is possible due to the gating property of the ReLU activations. Each path contains gates and weights, and the contribution of a path is the product of the gates and the weights in the path. We now discuss the role of gates in a DNN, by splitting them into i) \emph{active} gates which are `on' gates, and ii) \emph{sensitive} gates which are near $0$ and can flip from $0$ to $1$ or vice-versa based on gradient information.
\FloatBarrier
\begin{figure}[h]
\centering
%\begin{minipage}{0.75\columnwidth}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccc}
\includegraphics[scale=0.5]{figs/nn-subnet.png}
\includegraphics[scale=0.5]{figs/nnsoft.png}
\includegraphics[scale=0.6]{figs/der-gate.png}
%\includegraphics[scale=0.5]{figs/nnconv-size2.png}
%\includegraphics[scale=0.5]{figs/gradflow.png}
%\includegraphics[scale=0.5]{figs/nntwin-blck.png}
%\includegraphics[scale=0.5]{figs/nn.png}
%\includegraphics[scale=0.5]{figs/nn.png}
\end{tabular}
}
%\end{minipage}
%\begin{minipage}{0.18\columnwidth}
%\resizebox{\columnwidth}{!}{
%\includegraphics[scale=0.5]{figs/nnconv.png}
%}
%\end{minipage}
\caption{Illustration of the `path-view'.}
\label{fig:cartoon}
\end{figure}

\subsection{Active Gates and Capacity}
For each input example, a set of gates are \emph{on} in each layer, and this gives rise to the sub-network of active paths for that input. This active sub-network can be said to hold the memory for a given input (see cartoon $(b)$ in \Cref{fig:cartoon}), i.e., only those active paths that pass through the active gates contribute to the output. 

We note that, for DNNs with ReLU, with no bias parameters, a dataset with $n=2$ points namely $(x,1)$ and $(x/2,-1)$ for some $x\in \R^{d_{in}}$ cannot be memorised. The reason is that the gating values are the same for both $x$ and $x/2$ (for that matter any positive scaling of $x$), and hence $\phi_{x/2,\Theta}= \phi_{x,\Theta}/2$, and thus it not possible to fit arbitrary values for $\hat{y}_t(x/2)$ and $\hat{y}_t(x)$, since $\hat{y}_t(x/2)= \hat{y}_t(x)/2$. Cartoons $(a)$ and $(b)$ in \Cref{fig:cartoon} illustrate this scale invariance for inputs $x=(1,-1,2)\in\R^3$ and $x/2=(0.5,-0.5,1)\in\R^3$:  when compared to $(a)$, pre-activation values and output of $(b)$ are scaled down by a factor $2$, and the gating values of $(a)$ and $(b)$ are identical. \cite{ben} showed that DNNs can fit even random labels, and random pixels of standard datasets such as MNIST. However, it is clear from the above illustration that for any two inputs if their active sub-networks are similar, then their outputs cannot be arbitrarily different. 

Consider the deep linear network (DNLN), wherein, the activation is an identity function, which in turn can be thought of as a network whose gates are always on. Thus, all the paths are on for all the inputs, and the DLN can be reduced to a simple matrix. On the contrary, in a DNN with ReLU activations, different inputs will fire different sub-networks thereby increasing the capacity of such networks over DLNs.

\subsection{Sensitive Gates and Soft-ReLU} 
Consider the case of gates whose pre-activation inputs are near $0$, i.e., $\pm\epsilon$. Such gates are called sensitive gates, and during training, such gates can flip from $0$ to $1$ or vice-versa. Thus, by tuning such sensitive gates, gradient descent learns the right active sub-network for each input in the dataset. Note that, in the case of ReLU, the derivative of the gate is almost surely $0$, and hence it is not possible to capture the role of sensitive gates. We call this the ReLU artefact, which we remedy by considering a soft-ReLU activation, whose gating is given by $\gamma_{sr}(q)=\frac{1}{\left(1+\exp(-\beta \cdot q)\right)}, \beta>0$, and the activation is given by $\chi_{sr}(q)=q\cdot \gamma_{sr}(q)$. In the case of soft-ReLU, the derivative of the gating with respect to the pre-activation is given by $\partial_{q}\gamma_{sr}(q)=\frac{\beta}{\left(1+\exp(\beta\cdot q)\right)\left(1+\exp(-\beta\cdot q)\right)}$ (see rightmost plot in \Cref{fig:cartoon}).


==> npf.tex <==
\section{Neural Path Feature and Kernel: Encoding Gating Information}\label{sec:path}
First step in understanding the role of gates is to explicitly \emph{encode} the $1/0$ states of the gates. The gating property of the ReLU activation allows us to express the output of the DNN as a summation of the contribution of the individual paths, and paves a natural way to encode the $1/0$ states of the gates \emph{without loss of information}. The contribution of a path is the product of the signal in its input node, the weights in the path and the gates in the path. For an input $x\in\R^{\din}$, and parameter $\Theta\in\R^{\dnet}$, 
we encode the gating information in a novel \emph{neural path feature} (NPF), $\phi_{x,\Theta}\in\R^P$ and the weights in a novel \emph{neural path value} (NPV) $v_{\Theta}\in\R^P$, where $P$ is the total number of paths. 
The NPF co-ordinate of a path is the product of the signal at its input node and the gates in the path. The NPV co-ordinate of a path is the product of the weights in the paths. The output is then given by
\begin{align}\label{eq:npfnpv}
\hat{y}_{\Theta}(x)=\ip{\phi_{x,\Theta}, v_{\Theta}},
\end{align}
where $\phi_{x,\Theta}$ can be seen as the \emph{hidden features} which along with $v_{\Theta}$ are learned by gradient descent.
\begin{comment}
By stacking the NPFs of all the input examples we obtain the NPF matrix as $\Phi_{\Theta}=(\phi_{x_s,\Theta},s\in[n])\in\R^{P\times n}$. Then the input-output relationship of a DNN in vector form is given by:
\begin{align}\label{eq:npfnpv}
\hat{y}_{\Theta}=\Phi^\top_{\Theta} v_{\Theta},
\end{align}
where the NPF matrix $\Phi_{\Theta}$ can also be interpreted as the \emph{hidden feature matrix} which along with $v_{\Theta}$ is learnt during gradient descent on $\Theta\in\R^{\dnet}$. 
\end{comment}
\subsection{Paths, Neural Path Feature, Neural Path Value and Network Output}
We consider fully-connected DNNs with `$w$' hidden units per layer and `$d-1$' hidden layers where $\Theta\in\R^{\dnet}$ are the network weights ($\dnet=\din w+(d-2)w^2+w$). The information flow is show in \Cref{tb:basic}, where
$\Theta(i,j,l)$ is the weight connecting the $j^{th}$ hidden unit of layer $l-1$ to the $i^{th}$ hidden unit of layer $l$. Further, $\Theta(\cdot,\cdot,1)\in\R^{w\times \din}, \Theta(\cdot,\cdot,l)\in\R^{w\times w},\forall l\in\{2,\ldots,d-1\}, \Theta(\cdot,\cdot,d)\in\R^{1\times w}$.
\begin{table}[h]
\centering
\begin{tabular}{|c l lll|}\hline
Input Layer&: &$z_{x,\Theta}(0)$ &$=$ &$x$ \\
Pre-Activation Input&: & $q_{x,\Theta}(i,l)$& $=$ & $\sum_{j} \Theta(i,j,l)\cdot z_{x,\Theta}(j,l-1)$\\
Gating Values&: &$G_{x,\Theta}(i,l)$& $=$ & $\mathbbm{1}_{\{q_{x,\Theta}(i,l)>0\}}$\\
Hidden Layer. Output&: &$z_{x,\Theta}(i,l)$ & $=$ & $q_{x,\Theta}(i,l)\cdot G_{x,\Theta}(l,i)$ \\
Final Output&: & $\hat{y}_{\Theta}(x)$ & $=$ & $\sum_{j} \Theta(1,j,l)\cdot z_{x,\Theta}(j,d-1)$\\\hline
\end{tabular}
\caption{Here, $l\in[d-1],i\in[w]$, $j\in[\din]$ for $l=1$ and $j\in[w]$ for $l=d$.} 
\label{tb:basic}
\end{table}

\textbf{Paths:} A path starts from an input node, passes through exactly one weight (and one hidden node) in each layer and ends at the output node. We have a total of $P=\din w^{(d-1)}$ paths. We denote the set of all paths by $[P]$ (i.e., an enumeration). Let $\I_{l}\colon [P]\ra [w],l=1,\ldots,d-1$ provide the index of the hidden unit through which a path $p$ passes in layer $l$, and $\I_{0}\colon [P]\ra [\din]$ provides the input node.
\begin{definition}\label{def:nps} Let $x\in\R^{\din}$ be the input to the DNN. For this input, 

(i) The activity of a path $p$ is given by : $A_{\Theta}(x,p)\stackrel{def}{=}\Pi_{l=1}^{d-1} G_{x,\Theta}(l,\I_l(p))$.

(ii) The {neural path feature} (NPF) is given by :  $\phi_{x,\Theta}\stackrel{def}=\left(x(\I_0(p))A_{\Theta}(x_s,p) ,p\in[P]\right)\in\R^P$. 

(iii) The {neural path value} (NPV) if given by : $v_{\Theta}\stackrel{def}=\left(\Pi_{l=1}^d \Theta(l,\I_{l-1}(p),\I_l(p)),p\in[P]\right)\in\R^P$.
\end{definition}
\textbf{Remark:} A path $p$ is active if all the gates in the paths are on.
\begin{proposition}\label{prop:zero}  The output of the network can be written as an inner product of the NPF and NPV, i.e., 
$\hat{y}_{\Theta}(x)=\ip{\phi_{x,\Theta},v_{\Theta}}=\sum_{p\in [P]}x(\I_0(p))A_{\Theta}(x,p)v_{\Theta}(p)$.
\end{proposition}


==> npk.tex <==
\subsection{Neural Path Kernel : Similarity based on active sub-networks}
\begin{definition}\label{def:lambda}
 For input examples $s,s'\in[n]$, define $Act_{\Theta}(s,s')\stackrel{def}=\{p\in[P]\colon A_{\Theta}(x_s,p)= A_{\Theta}(x_{s'},p)=1\}$ to be the set of `active' paths for both $s,s'$  and $\Lambda_{\Theta}(s,s')\stackrel{def}=\frac{|Act_{\Theta}(s,s')|}{\din}$.
\end{definition}
\textbf{Remark:} Owing to the symmetry of a DNN, the same number of active paths start from any fixed input node. In \Cref{def:lambda}, $\Lambda_{\Theta}$ measures the size of the active sub-network as the total number of active paths starting from any fixed input node. For examples $s,s'\in[n],s\neq s'$, $\Lambda_{\Theta}(s,s)$ is equal to the size of the sub-network active for $s$, and $\Lambda_{\Theta}(s,s')$ is equal to the size of the sub-network active for both $s$ and $s'$. For an illustration of NPFs and $\Lambda$ please see \Cref{fig:npkexample}.
\begin{lemma}\label{lm:npk}
Let $H_{\Theta}\in\R^{n\times n}$ be the NPK matrix, whose entries are given by $H_{\Theta}(s,s')\stackrel{def}{=}\ip{\phi_{x_s,\Theta},\phi_{x_{s'},\Theta}},s,s'\in[n]$. Let $\Sigma\in\R^{n\times n}$ be the input Gram matrix with entires $\Sigma(s,s')=\ip{x_s,x_{s'}},s,s'\in[n]$. It follows that $H_{\Theta}= \Sigma\odot\Lambda_{\Theta}$, where $\odot$ is  the Hadamard product.
\end{lemma}


==> npkexample.tex <==
\FloatBarrier
\begin{figure}[h]
\centering
\resizebox{\columnwidth}{!}{
\includegraphics[scale=1]{figs/npf-npk.png}
}
\centering
\begin{minipage}{0.64\textwidth}
\resizebox{\columnwidth}{!}{
$\phi_{x_1}=[0, 0, x_1(1),0,0, 0, 0,0, x_1(1), 0, 0, x_1(2),0, 0, 0,0, 0, x_1(2)]^\top$
}
\\
\resizebox{\columnwidth}{!}{
$\phi_{x_2}=[0, x_2(1), x_2(1),0,0, 0, 0,0,0, 0, x_2(2), x_2(2),0,0, 0, 0,0,0 ]^\top$
}
\\
\resizebox{\columnwidth}{!}{
$\phi_{x_3}=[0, 0,0,0, x_3(1),x_3(1),0,0, 0,0, 0,0,0, x_3(2),x_3(2),0,0, 0 ]^\top$
}
\end{minipage}
\begin{minipage}{0.25\textwidth}
,\,$\Lambda=\left[\begin{matrix} 
2 &1& 0 \\
1 &2& 0\\
0 &0& 2
\end{matrix}\right]$
\end{minipage}
\caption{A toy illustration of gates, paths and active sub-networks. The cartoon (\textbf{a}) in the top left corner shows a DNN with $2$ hidden layers, $6$ ReLU gates $G(l,i),l=1,2,i=1,2,3$, $2$ input nodes $x(1)$ and $x(2)$ and an output node $\hat{y}_{\Theta}(x)$. Cartoons (\textbf{b}) to (\textbf{g}) show the enumeration of the paths $p_1,\ldots, p_{18}$. Cartoons (\textbf{h}), (\textbf{i}) and (\textbf{j}) show hypothetical gates for $3$ different hypothetical input examples $\{x_s\}_{s=1}^3 \in\R^2$. In each of the cartoons (\textbf{h}), (\textbf{i}) and (\textbf{j}), the $1/0$ inside the circles denotes the on/off state of the gates, and the bold paths/gates shown in red colour constitute the active sub-network for that particular input example. The NPFs are given by $\phi_{x}=[x(1)A(x,p_1),\ldots,x(1)A(x,p_{9}),x(2)A(x,p_{10}),\ldots,x(2)A(x,p_{18})]^\top$. Here, $\Lambda(1,2)=1$ because paths $p_3$ and $p_{12}$ are both active for input examples $x_1$ and $x_2$ and the input dimension is $2$.}
\label{fig:npkexample}
\end{figure}



==> related.tex <==
\section{Related Work}
\setcitestyle{authoryear}
\textbf{Gated Linear Unit (GaLU)} networks with single hidden layer was theoretically analysed by \cite{sss,fiat}. A critical difference between our work and that of \cite{sss,fiat} is that our NPFs/NPV formulation enabled us to analyse DGNs of any depth $d$. The fixed random filter setting of \cite{fiat} is equivalent to (in our setting) FRNPF for DGNs with single hidden layer. They test the hypothesis (on MNIST and Fashion-MNIST) that the effectiveness of ReLU networks is mainly due to the training of the linear part (i.e., weights) and not the gates. They also show that a ReLU network marginally outperforms a GaLU network (both networks have a single hidden layer), and propose a non-gradient based \textbf{Algorithm 1} (which has a separate loop to randomly search and replace the gates of the GaLU network) to close the margin between the GaLU and ReLU networks. We observe a similar trend in that, the FRNPFs (here only NPV is learnt) do perform well in the experiments with a test accuracy of around $68\%$ on CIFAR-10. However, it is also the case that models with NPF learning perform significantly better (by more than $10\%$) than FRNPF, which underscores the importance of the gates. Further, we used soft-ReLU gates in the DLNPF regime, and showed that using standard optimisers (gradient descent based), we can learn the NPFs and NPV in two separate networks. In addition, capturing the role of the active sub-networks via the NPK is another significant progress over \cite{sss,fiat}.% resulting better generalisation than learning only NPV keeping the NPFs fixed and random. %We believe that handling of depth $d$ networks, identification and the use of novel quantities namely NPFs, NPK and, the role of NPF learning in generalisation amount to significant progress in comparison to \cite{sss}. 
%as opposed to only single hidden layer GaLU networks handled by \cite{sss,fiat}. 

\textbf{Prior NTK works:} \cite{ntk} showed the NTK to be the central quantity in the study of generalisation properties of infinite width DNNs. \cite{jacot2019freeze} identify two regimes that occur at initialisation in fully connected DNNs as the width increases to infinity namely i) \emph{freeze:} here, the (scaled) NTK converges to a constant and hence leads to slow training,  and  ii) \emph{chaos:} here, the NTK converges to Kronecker delta and hence hurts generalisation. \cite{jacot2019freeze} also suggest that for good generalisation it is important to operate the DNNs at the edge of the freeze and the chaos regimes. The works of \cite{arora2019exact,cao2019generalization} are closely related and has been discussed in the introduction.
\cite{dudnn} use the NTK to show that over-parameterised DNNs trained by gradient descent achieve zero training error. \cite{dudln,shamir,ganguli} studied deep linear networks (DLNs). Since DLNs are special cases of DGNs, \Cref{th:main} of our paper also provides an expression for the NTK at initialisation of deep linear networks. To see this, in the case of DLNs, all the gates are always $1$ and $\Lambda_{\Theta}$ is a matrix whose entries will be $w^{(d-1)}$. %The results in our paper are complementary to the prior NTF/NTK based works, in that, the NPK and NPFs are zeroth order kernel and features respectively. In contrast, the NTF is the gradient of the network output with respect to the weights of the network and hence the NTF/NTK are essentially first order quantities. In the fixed NPF setting the gates are explicitly controlled by a separate feature network, an aspect is absent in prior works.


%\cite{arora2019exact} proposed pure kernel method based on the infinite width CNTK (NTK of convolutional neural network) and showed that it out performed state-of-the-art kernel methods by $10\%$. \cite{arora2019exact} also noted a performance gain (about $5-6\%$) of the CNNs over the CNTK.  However, it was also noted by \cite{arora2019exact,lee2019wide} that random NTFs obtained from finite width neural networks do not perform as well as their limiting infinite width counterparts. 
%\cite{arora,cao2019generalization} provided generalisation bounds with the NTK norm.

%\begin{comment}

%\end{comment}

\textbf{Other works:} Empirical analysis of the role of gates was done by \cite{srivastava2014understanding}, where the active sub-networks are called as \emph{locally competitive} networks. Here, a `sub-mask' encodes the $0/1$ state of the all the gates. A t-SNE visualisation of the sub-masks showed that the ``subnetworks active for examples of the same class are much more similar to each other compared to the ones activated for the examples of different classes''. \cite{balestriero2018spline}  connect $\max$-affine linearity and DNN with ReLU activations. \cite{neyshabur2015path} proposed a novel \emph{path-norm} based gradient descent. 



==> varproof_bkp.tex <==

\begin{proposition}
For a path $p\in[P]$ and let $\phi_{p,\Tv}\eqdef \left(\partial_{\tv} v_{\Tv}(p), \tv\in\Tv\right)\in\R^{\dvnet}$. Let $\tv\in\Tv$ be any arbitrary weight in layer $l'$, then 

(i) $\phi_{p,\Tv}(\tv) = 0$, if the path $p$ does not pass through $\tv$.


(ii) $\phi_{p,\Tv}(\tv) = \Pi_{l=1,l\neq l'}^{(d-1)}\Theta(\I_{l-1}(p),\I_l(p),l)$.
\end{proposition}

\begin{proof}
Proof follows by noting that $v_{\Tv}(p)=\Pi_{l=1}^{(d-1)}\Theta(\I_{l-1}(p),\I_l(p),l)$, and that the said arbitrary weight $\tv$ in layer $l'$.
\end{proof}


For $x,x'\in\R^{\din}$, let $f_{\Tf}(p)=x(\I_0(p)) A_{\Tf}(x,p)$. and $f'_{\Tf}(p)=x'(\I_0(p)) A_{\Tf}(x',p)$ Then we have
\begin{align*}
\hat{y}_{\Tdgn}(x)= \sum_{p\in[P]} f_{\Tf}v_{\Tv}(p)
\end{align*}
Let $\tv\in\Tv$, and $\partial_{\tv}(\cdot)$ denote $\frac{\partial (\cdot)}{\partial \tv}$.  Then,
\begin{align*}
\partial_{\tv}\hat{y}{\Tdgn}(x)&= \sum_{p\in[P]} f_{\Tf}\partial v_{\Tv}(p)
\nabla_{\Tv}\hat{y}_{\Tdgn}(x) &= \left(\partial_{\tv}\hat{y}_{\Tdgn}(x),\tv\in\Tv\right)\in\R^{\dvnet}
\end{align*}
From now on we drop $\Tdgn$ from $f_{\Tdgn}$ and, $\hat{y}_{\Tdgn}$ and drop $\Tv$ from $v_{\Tv}$ and $\nabla_{\Tv}$. 
\begin{align}
\ip{\nabla \hat{y}(x), \hat{y}(x')}=\sum_{\ta}\left(\sum_{p_a}f(p_a) \partial_{\ta}v(p_a) \right)\left(\sum_{p'_a}f'(p'_a) \partial_{\ta}v(p'_a) \right)
\end{align}

\begin{align*}
K(x,x') 	&= \sum_{\ta,p_a,p'_a} f(p_a) f'(p'_a) \partial_{\ta}v(p_a) \partial_{\ta}v(p'_a) \\
\E{K(x,x')} 	&= \sum_{\ta,p_a} f(p_a) f'(p_a) \E{\left(\partial_{\ta}v(p_a)\right)^2}
\end{align*}

\begin{align}
\E{K(x,x')}^2 = \underset {\tb,p_b}{\underset{\ta,p_a}{\sum}} f(p_a) f'(p_a) f(p_b) f'(p_b) \E{\left(\pta v(p_a)\right)^2}\E{\left(\ptb v(p_b)\right)^2}
\end{align}

\begin{align}
K^2(x,x')= \underset {\tb,p_b,p'_b}{\underset{\ta,p_a,p'_a} {\sum}} f(p_a) f'(p'_a) f(p_b) f'(p'_b) \pta v(p_a) \pta v(p'_a) \ptb v(p_b) \ptb v(p'_b)
\end{align}

\begin{align}
\E{K^2(x,x')}= \underset {\tb,p_b,p'_b}{\underset{\ta,p_a,p'_a} {\sum}} f(p_a) f'(p'_a) f(p_b) f'(p'_b)\E{ \pta v(p_a) \pta v(p'_a) \ptb v(p_b) \ptb v(p'_b)}
\end{align}

\begin{proposition} \label{prop:prod}
Let $\ta$ belong to layer $l_a\in[d-1]$ and $\tb\in[d-1]$ belong to layer $l_b$. Let paths $p_a$ and $p'_a$ pass through $\ta$ and paths $p_b$ and $p'_b$ pass through $\tb$. Let $E(p_a,p'_a,p_b,p'_b; \ta,\tb) = \E{ \pta v(p_a) \pta v(p'_a) \ptb v(p_b) \ptb v(p'_b)}$, then 
\small
\begin{align*}
&E(p_a,p'_a,p_b,p'_b; \ta,\tb)\\ 
			=&\underbrace{\underset{l\neq \l_a}{\underset{l\neq \l_b} {\underset{l=1}{\Pi^{(d-1)}}}}  \E{\Theta(\I_{l-1}(p_a),\I_l(p_a),l )\Theta(\I_{l-1}(p'_a),\I_l(p'_a),l )\Theta(\I_{l-1}(p_b),\I_l(p_b),l )\Theta(\I_{l-1}(p'_b),\I_l(p'_b),l )}}_{\text{Term-I}}\\
		      	&\underbrace{\cdot\E{ \Theta(\I_{l_b-1}(p_a),\I_{l_b}(p_a),l_b )\Theta(\I_{l_b-1}(p'_a),\I_{l_b}(p'_a),l_b) }}_{\text{Term-II}}\\
		      	&\underbrace{\cdot \E{\Theta(\I_{l_a-1}(p_b),\I_{l_a}(p_b),l_a )\Theta(\I_{l_a-1}(p'_b),\I_{l_a}(p'_b),l_a)}}_{\text{Term-III}}
\end{align*}
\end{proposition}
\begin{proof}
\normalsize
Expand the individual terms  $\pta v(p_a)$, $\pta v(p'_a)$,  $\ptb(p_b)$ and $\ptb(p'_b)$ in $E(p_a,p'_a,p_b,p'_b; \ta,\tb)$. We have
\begin{align*}
\pta v(p_a) =& \Pi_{l=1,l\neq l_a}^{(d-1)} \Theta(\I_{l-1}(p_a),\I_{l}(p_a),l )\\
\pta v(p'_a) =& \Pi_{l=1,l\neq l_a}^{(d-1)} \Theta(\I_{l-1}(p'_a),\I_{l}(p'_a),l )\\
\pta v(p_b) =& \Pi_{l=1,l\neq l_b}^{(d-1)} \Theta(\I_{l-1}(p_b),\I_{l}(p_b),l )\\
\pta v(p'_b) =& \Pi_{l=1,l\neq l_b}^{(d-1)} \Theta(\I_{l-1}(p'_b),\I_{l}(p'_b),l )\\
\end{align*}
The proof is complete by using the fact that weights of different layers are independent and pushing the $\mathbb{E}$ operator inside the $\E{ \pta v(p_a) \pta v(p'_a) \ptb v(p_b) \ptb v(p'_b)}$ to convert the expectation of products into a product of expectations.
\end{proof}


\begin{comment}
\begin{proposition} \label{prop:prod}
Let $\ta$ belong to layer $l_a\in[d-1]$ and $\tb\in[d-1]$ belong to layer $l_b$. Let paths $p_a$ and $p'_a$ pass through $\ta$ and paths $p_b$ and $p'_b$ pass through $\tb$. Let $E(p_a,p'_a,p_b,p'_b; \ta,\tb) = \E{ \pta v(p_a) \pta v(p'_a) \ptb v(p_b) \ptb v(p'_b)}$, then 

(i) If $l_a=l_b$, then 
\small
\begin{align*}
&E(p_a,p'_a,p_b,p'_b; \ta,\tb)\\
=&\underbrace{\Pi_{l=1,l\neq l_a}^{(d-1)} \E{\Theta(\I_{l-1}(p_a),\I_l(p_a),l )\Theta(\I_{l-1}(p'_a),\I_l(p'_a),l )\Theta(\I_{l-1}(p_b),\I_l(p_b),l )\Theta(\I_{l-1}(p'_b),\I_l(p'_b),l )}}_{\text{Term-I}}
\end{align*}
\normalsize
(ii) If $l_a\neq l_b$, then 
\small
\begin{align*}
&E(p_a,p'_a,p_b,p'_b; \ta,\tb)\\ 
			=&\underbrace{\underset{l\neq \l_a}{\underset{l\neq \l_b} {\underset{l=1}{\Pi^{(d-1)}}}}  \E{\Theta(\I_{l-1}(p_a),\I_l(p_a),l )\Theta(\I_{l-1}(p'_a),\I_l(p'_a),l )\Theta(\I_{l-1}(p_b),\I_l(p_b),l )\Theta(\I_{l-1}(p'_b),\I_l(p'_b),l )}}_{\text{Term-I}}\\
		      	&\underbrace{\cdot\E{ \Theta(\I_{l_b-1}(p_a),\I_{l_b}(p_a),l_b )\Theta(\I_{l_b-1}(p'_a),\I_{l_b}(p'_a),l_b) }}_{\text{Term-II}}\\
		      	&\underbrace{\cdot \E{\Theta(\I_{l_a-1}(p_b),\I_{l_a}(p_b),l_a )\Theta(\I_{l_a-1}(p'_b),\I_{l_a}(p'_b),l_a)}}_{\text{Term-III}}
\end{align*}
\end{proposition}
\begin{proof}
\normalsize
Expand the individual terms  $\pta v(p_a)$, $\pta v(p'_a)$,  $\ptb(p_b)$ and $\ptb(p'_b)$ in $E(p_a,p'_a,p_b,p'_b; \ta,\tb)$. We have
\begin{align*}
\pta v(p_a) =& \Pi_{l=1,l\neq l_a}^{(d-1)} \Theta(\I_{l-1}(p_a),\I_{l}(p_a),l )\\
\pta v(p'_a) =& \Pi_{l=1,l\neq l_a}^{(d-1)} \Theta(\I_{l-1}(p'_a),\I_{l}(p'_a),l )\\
\pta v(p_b) =& \Pi_{l=1,l\neq l_b}^{(d-1)} \Theta(\I_{l-1}(p_b),\I_{l}(p_b),l )\\
\pta v(p'_b) =& \Pi_{l=1,l\neq l_b}^{(d-1)} \Theta(\I_{l-1}(p'_b),\I_{l}(p'_b),l )\\
\end{align*}
The proof is complete by using the fact that weights of different layers are independent and pushing the $\mathbb{E}$ operator inside the $\E{ \pta v(p_a) \pta v(p'_a) \ptb v(p_b) \ptb v(p'_b)}$ to convert the expectation of products into a product of expectations.
\end{proof}
\end{comment}


\begin{proposition}[Necessary Conditions for Survival]\label{lm:necc}
Let $p_a,p'_a,p_b,p'_b$ be $4$ arbitrary paths, and let $\ta$ and $\tb$ be two arbitrary weights. Let $\ta$ belong to layer $l_a\in[d-1]$ and let $\tb$ belong to layer $l_b\in[d-1]$. Then $E(p_a,p'_a,p_b,p'_b; \ta,\tb)\neq 0$ only if 

$\bullet$ \textbf{Condition I:} In all the $3$ cases $p_a, p'_a$ pass through $\ta$ \emph{and} $p_b, p'_b$ pass through $\tb$.

$\bullet$ \textbf{Condition II:} In every layer, $l\in[d]$ either all the $4$ paths $p_a,p'_a,p_b,p'_b$ pass through the same weight \emph{or} there exists two distinct weights, say $\theta_{\text{I},l}$ and $\theta_{\text{II},l}$ such that, $2$ paths out of $p_a,p'_a,p_b,p'_b$ pass through $\theta_{\text{I},l}$ and the other two through $\theta_{\text{II},l}$.

\end{proposition}

\begin{proof}
If \textbf{Condition I} does not hold, then either one of $\pta v(p_a), \pta v(p'_a), \ptb v(p_b), \ptb v(p'_b)$ becomes $0$. 
If \textbf{Condition II} does not hold, either Term-I or Term-II or Term-III in \Cref{prop:prod} evaluates to $0$ because all the weights involved are symmetric Bernoulli.
\end{proof}



\begin{comment}
\begin{proposition}[Necessary Conditions for Survival]\label{lm:necc}
Let $p_a,p'_a,p_b,p'_b$ be $4$ arbitrary paths, and let $\ta$ and $\tb$ be two arbitrary weights. Let $\ta$ belong to layer $l_a\in[d-1]$ and let $\tb$ belong to layer $l_b\in[d-1]$. Let us consider $3$ cases namely \emph{Case A:} $\ta=\tb$, \emph{Case B:}$\ta\neq\tb$ and $l_a=l_b$ \emph{Case C:} $\ta\neq\tb$ and $l_a\neq l_b$. Let $E(p_a,p'_a,p_b,p'_b; \ta,\tb)$ be in \Cref{prop:prod}, then  \textbf{Condition} I and \textbf{Condition II} given below are necessary for the survival of of $E(p_a,p'_a,p_b,p'_b; \ta,\tb)$, i.e., for $E(p_a,p'_a,p_b,p'_b; \ta,\tb)\neq 0$. 

$\bullet$ \textbf{Condition I:} In all the $3$ cases $p_a, p'_a$ pass through $\ta$ \emph{and} $p_b, p'_b$ pass through $\tb$.

$\bullet$ \textbf{Condition II:} 

\indent\,\,For \emph{Case A and B:} Let $\ta(=\tb)$ belong to layer $l_{ab}(=l_a=l_b)$. For $l\neq l_{ab}$, (i) all the $4$ paths namely $p_a,p'_a,p_b,p'_b$ pass through a weight $\theta_{\text{I},l}$ \emph{or} (ii) $2$ out of the $4$ paths namely $p_a,p'_a,p_b,p'_b$ pass through a weight $\theta_{\text{I},l}$ belonging to a layer $l$ and the other $2$ paths pass through another weight $\theta_{\text{II},l}$ belonging to a layer $l$.

\indent\,\,For \emph{Case C:}  

\indent\,\,\quad\quad	$1.$ For $l\neq l_{a}, l\neq l_b$ (i) all the $4$ paths namely $p_a,p'_a,p_b,p'_b$ pass through a weight $\theta_{\text{I},l}$ belonging to layer $l$ \emph{or} (ii) $2$ out of the $4$ paths namely $p_a,p'_a,p_b,p'_b$ pass through a weight $\theta_{\text{I},l}$ belonging to a layer $l$ and the other $2$ paths pass through another weight $\theta_{\text{II},l}$ belonging to a layer $l$.
\begin{center}
\emph{and}
\end{center}
\indent\,\,\quad\quad	$2.$ For $l= l_{a}$ (i) all the $4$ paths namely $p_a,p'_a,p_b,p'_b$ pass through a weight $\ta$ \emph{or} (ii) paths $p_b,p'_b$ pass through a weight $\theta_{\text{I},l}$ (different from $\ta$) belonging to a layer $l$.
\begin{center}
\emph{and}
\end{center}
\indent\,\,\quad\quad	$3.$ For $l= l_{b}$ (i) all the $4$ paths namely $p_a,p'_a,p_b,p'_b$ pass through a weight $\tb$ \emph{or} (ii) paths $p_a,p'_a$ pass through a weight $\theta_{\text{I},l}$ (different from $\tb$) belonging to a layer $l$.
\end{proposition}

\begin{proof}
If \textbf{Condition I} does not hold, then either one of $\pta v(p_a), \pta v(p'_a), \ptb v(p_b), \ptb v(p'_b)$ becomes $0$. 

\textbf{Condition II} uses the fact that all the random variables are iid symmetric Bernoulli, and in simple terms states that i) when $4$ weights are picked from a given layer ($l\neq l_{ab}$ in \emph{Case A and Case B} and $l\neq l_{a}, \l \neq l_b$ in \emph{Case C}), for the expectation of the product of those weights to be non-zero, then either all $4$ are identical or they occur in pairs,  i.e., out of the $4$ weights there $2$  distinct and they repeat twice, or ii) when $2$ weights are picked from a layer ($l=l_a$ or $l=l_b$ in \emph{Case C}) then they should be identical. 

If \textbf{Condition II} does not hold, either Term-I or Term-II or Term-III in \Cref{prop:prod} evaluates to $0$ because all the weights involved are symmetric Bernoulli.
\end{proof}
\end{comment}

\begin{lemma}[Base Path Identification]
For any term $E(p_a,p'_a,p_b,p'_b;\ta,\tb)\neq 0$, it follows that there exists `\emph{base}' paths $\rho_a$ and $\rho_b$ such that 

(i) $\rho_a$ and $\rho_b$ pass through $\ta$ and $\tb$ respectively.

(ii) $E(p_a,p'_a,p_b,p'_b;\ta,\tb)= E(\rho_a,\rho_a,\rho_b,\rho_b;\ta,\tb)$.
\end{lemma}

\begin{proof}
Using \Cref{lm:necc} and the fact that $p_a,p'_a,p_b,p'_b$ are paths, only the following layouts are possible.
\FloatBarrier
\begin{figure}[h]
\centering
\resizebox{\columnwidth}{!}{
\includegraphics[scale=0.1]{figs/pathcases.png}
}
\end{figure}
\begin{center}
\begin{tabular}{|c|c|}\hline
Current Layer Layout & Next Layer Layout\\\hline
\textbf{(a)} &  \textbf{(a)} or  \textbf{(b)}\\\hline
\textbf{(b)} &  \textbf{(c)} or  \textbf{(d)}\\\hline 
\textbf{(c)} &  \textbf{(a)} or  \textbf{(b)}\\\hline 
\textbf{(d)} &  \textbf{(c)} or  \textbf{(d)}\\\hline 
\end{tabular}
\end{center}
\end{proof}

\begin{definition}\label{def:cross}
Paths $\rho_a$ and $\rho_b$ are said to cross each other if they pass through the same hidden node in one or many of the intermediate layers $l\in\{2,\ldots, d-1\}$. 
\end{definition}

\begin{

\begin{proposition}
Let $\rho_a$ and $\rho_b$ be base paths that cross at $k\in\{1,\ldots,d-1\}$ intermediate nodes, and let $S=\{(p_a,p'_a,p_b,p'_b) | \}$
\end{proposition}

\begin{theorem}
\end{theorem}
\begin{proof}
Note that for symmetric Bernoulli distribution $\E{\theta^2}^2=\E{\theta^4}=\sigma^4$. So,
\begin{align*}
&f(p_a) f'(p_a) f(p_b) f'(p_b) \E{\left(\pta v(p_a)\right)^2}\E{\left(\ptb v(p_b)\right)^2} \\
&= f(p_a) f'(p_a) f(p_b) f'(p_b)E(p_a,p_a,p_b,p_b;\ta,\tb)\\
&= f(p_a) f'(p_a) f(p_b) f'(p_b)\sigma^{4(d-1)}
\end{align*}
Thus, all the terms in the expansion of $\E{K(x,x')}^2$ are also in $\E{K^2(x,x')}$ and hence are not part of the variance expression, $Var\left[K(x,x')\right]=\E{K^2(x,x')}-\E{K(x,x')}^2$.

\end{proof}



